Elastic waves generated by impact and vibration in confined granular media

Observational data of asteroids can be explained by considering them as an agglomerate of granular material. Understanding the mechanical properties of these objects is relevant for many scientific reasons: space missions design, evaluation of impact threats to our planet, and understanding the nature of asteroids and their implication in the origin of the solar system. In-situ measurements of mechanical properties require complex and costly space missions. Here a laboratory-scale characterization of wave propagation in granular media is presented using a novel experimental setup as well as numerical simulations. The pressure inside an asteroid is still a matter of debate, but it definitely presents a pressure gradient towards the interior. This is why impact characterization needs to be performed as a function of the confining pressure. Our experimental setup allows for the simultaneous measurement of the external confining pressure, internal pressure, total strain, and acceleration in a 50 cm side squared box filled up with a billion grains. We study the propagation of impact-generated and shaker-born seismic body waves in the 500 Hz range. Through subsequent compression-relaxation cycles, it was observed that the granular media behaves on average like a solid with a constant elastic modulus during each compression. Effective medium theory (EMT) for granular media explains the data at low pressure. After each compression-relaxation cycle, the elastic modulus increases, and a high hysteresis is observed: relaxation shows a more complex behavior than compression. We show that seismic waves generated by both impact and vibration travels at the pressure wave speed. Thanks to a numerical model, we measure a strong wave attenuation $\alpha\sim3.4$ Np/m. We found that the wave speed increases with the confining pressure with a $p^{1/2}$.

==> BiblioNotUsed.tex <==
@article{dafalias1977cyclic,
  title={Cyclic loading for materials with a vanishing elastic region},
  author={Dafalias, Yannis F and Popov, Egor P},
  journal={Nuclear engineering and design},
  volume={41},
  number={2},
  pages={293--302},
  year={1977},
  publisher={Elsevier}
}

@article{sessarego2008frequency,
  title={Frequency dependence of phase speed, group speed, and attenuation in water-saturated sand: Laboratory experiments},
  author={Sessarego, Jean-Pierre and Ivakin, Anatoly N and Ferrand, Didier},
  journal={IEEE journal of oceanic engineering},
  volume={33},
  number={4},
  pages={359--366},
  year={2008},
  publisher={IEEE}
}

@article{bergamo2014physical,
  title={Physical modelling of a surface-wave survey over a laterally varying granular medium with property contrasts and velocity gradients},
  author={Bergamo, Paolo and Bodet, Ludovic and Socco, Laura Valentina and Mourgues, R{\'e}gis and Tournat, Vincent},
  journal={Geophysical Journal International},
  volume={197},
  number={1},
  pages={233--247},
  year={2014},
  publisher={Oxford University Press}
}

@article{Brum2019,
  title = {Drastic slowdown of the Rayleigh-like wave in unjammed granular suspensions},
  author = {Brum, Javier and Gennisson, Jean Luc and Fink, Mathias and Tourin, Arnaud and Jia, Xiaoping},
  journal = {Phys. Rev. E},
  volume = {99},
  issue = {4},
  pages = {042902},
  numpages = {9},
  year = {2019},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.99.042902},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.99.042902}
}


@Article{agnolin2008elastic,
  Title                    = {On the elastic moduli of three-dimensional assemblies of spheres: Characterization and modeling of fluctuations in the particle displacement and rotation},
  Author                   = {Agnolin, Ivana and Roux, J-N},
  Journal                  = {International Journal of Solids and Structures},
  Year                     = {2008},
  Number                   = {3-4},
  Pages                    = {1101--1123},
  Volume                   = {45},

  Publisher                = {Elsevier}
}

@Article{Akella2018,
  Title                    = {Force distributions in frictional granular media},
  Author                   = {Akella, VS and Bandi, MM and Hentschel, H George E and Procaccia, Itamar and Roy, Saikat},
  Journal                  = {Physical Review E},
  Year                     = {2018},
  Number                   = {1},
  Pages                    = {012905},
  Volume                   = {98},

  File                     = {:Biblio/Force Distribution in a Granular Medium.pdf:PDF},
  Publisher                = {APS}
}

@Misc{Amon2017preface,
  Title                    = {Preface: Focus on imaging methods in granular physics},

  Author                   = {Amon, Axelle and Born, Philip and Daniels, Karen E and Dijksman, Joshua A and Huang, Kai and Parker, David and Schr{\"o}ter, Matthias and Stannarius, Ralf and Wierschem, Andreas},
  Year                     = {2017},

  Journal                  = {Review of Scientific Instruments},
  Number                   = {5},
  Pages                    = {051701},
  Publisher                = {AIP Publishing LLC},
  Volume                   = {88}
}

@Article{catheline2022gravitational,
  Title                    = {Gravitational lens effect revisited through membrane waves},
  Author                   = {Catheline, Stefan and Delattre, Victor and Laloy-Borgna, Gabrielle and Faure, Fr{\'e}deric and Fink, Mathias},
  Journal                  = {American Journal of Physics},
  Year                     = {2022},
  Number                   = {1},
  Pages                    = {47--50},
  Volume                   = {90},

  Publisher                = {American Association of Physics Teachers}
}

@Article{domenico1977effect,
  Title                    = {Effect of brine-gas mixture on velocity in an unconsolidated sand reservoir},
  Author                   = {Domenico, SN},
  Journal                  = {The Log Analyst},
  Year                     = {1977},
  Number                   = {03},
  Volume                   = {18},

  Publisher                = {OnePetro}
}


@Article{duffaut2010using,
  Title                    = {Using Mindlin theory to model friction-dependent shear modulus in granular media},
  Author                   = {Duffaut, Kenneth and Landr{\o}, Martin and Sollie, Roger},
  Journal                  = {Geophysics},
  Year                     = {2010},
  Number                   = {3},
  Pages                    = {E143--E152},
  Volume                   = {75},

  Publisher                = {Society of Exploration Geophysicists}
}

@Article{Glavatskiy2006,
  Title                    = {$\backslash$mu $-model for the statics of dry granular medium},
  Author                   = {Glavatskiy, KS and Kulinskii, VL},
  Journal                  = {arXiv preprint cond-mat/0603565},
  Year                     = {2006}
}

@Article{Han2016high,
  Title                    = {High-speed ultrasound imaging in dense suspensions reveals impact-activated solidification due to dynamic shear jamming},
  Author                   = {Han, Endao and Peters, Ivo R and Jaeger, Heinrich M},
  Journal                  = {Nature communications},
  Year                     = {2016},
  Number                   = {1},
  Pages                    = {1--8},
  Volume                   = {7},

  Publisher                = {Nature Publishing Group}
}

@Article{Jannsen1895,
  Title                    = {Verrsuche uber quetreidedruck in silozellen},
  Author                   = {Jannsen, HA},
  Journal                  = {Z. Ver. Dtsch. Ing},
  Year                     = {1895},
  Pages                    = {1045--1049},
  Volume                   = {39}
}

@Article{jannsen1895verrsuche,
  Title                    = {Verrsuche uber quetreidedruck in silozellen},
  Author                   = {Jannsen, HA},
  Journal                  = {Z. Ver. Dtsch. Ing},
  Year                     = {1895},
  Pages                    = {1045--1049},
  Volume                   = {39}
}

@InProceedings{jespersen1998ultrasound,
  Title                    = {Ultrasound spatial compound scanner for improved visualization in vascular imaging},
  Author                   = {Jespersen, S{\o}ren Kragh and Wilhjelm, Jens E and Sillesen, H},
  Booktitle                = {1998 IEEE Ultrasonics Symposium. Proceedings (Cat. No. 98CH36102)},
  Year                     = {1998},
  Organization             = {IEEE},
  Pages                    = {1623--1626},
  Volume                   = {2}
}

@Article{jia1999ultrasound,
  Title                    = {Ultrasound propagation in externally stressed granular media},
  Author                   = {Jia, Xiaoping and Caroli, C and Velicky, B},
  Journal                  = {Physical Review Letters},
  Year                     = {1999},
  Number                   = {9},
  Pages                    = {1863},
  Volume                   = {82},

  Publisher                = {APS}
}

@Article{lorenzo2013benchmark,
  Title                    = {Benchmark hydrogeophysical data from a physical seismic model},
  Author                   = {Lorenzo, Juan M and Smolkin, David E and White, Christopher and Chollett, Shannon R and Sun, Ting},
  Journal                  = {Computers \& Geosciences},
  Year                     = {2013},
  Pages                    = {44--51},
  Volume                   = {50},

  Publisher                = {Elsevier}
}

@Article{mashinsky2003,
  Title                    = {Differences between static and dynamic elastic moduli of rocks: Physical causes},
  Author                   = {Mashinsky, EI},
  Journal                  = {Russian Geology and Geophysics},
  Year                     = {2003},
  Number                   = {9},
  Pages                    = {953--959},
  Volume                   = {44}
}

@Article{quillen2022propagation,
  Title                    = {Propagation and attenuation of pulses driven by low velocity normal impacts in granular media},
  Author                   = {Quillen, AC and Neiderbach, Max and Suo, Bingcheng and South, Juliana and Wright, Esteban and Skerrett, Nathan and S{\'a}nchez, Paul and C{\'u}{\~n}ez, Fernando David and Miklavcic, Peter and Askari, Heesam},
  Journal                  = {arXiv preprint arXiv:2201.01225},
  Year                     = {2022}
}

@Article{sperl2006experiments,
  Title                    = {Experiments on corn pressure in silo cells--translation and comment of Janssen's paper from 1895},
  Author                   = {Sperl, Matthias},
  Journal                  = {Granular Matter},
  Year                     = {2006},
  Number                   = {2},
  Pages                    = {59--65},
  Volume                   = {8},

  Publisher                = {Springer}
}

@Article{yang2016shear,
  Title                    = {Shear wave velocity and stiffness of sand: the role of non-plastic fines},
  Author                   = {Yang, J and Liu, X},
  Journal                  = {G{\'e}otechnique},
  Year                     = {2016},
  Number                   = {6},
  Pages                    = {500--514},
  Volume                   = {66},

  Publisher                = {Thomas Telford Ltd}
}


